Graph Federated Learning with Hidden Representation Sharing

Learning on Graphs (LoG) is widely used in multi-client systems when each client has insufficient local data, and multiple clients have to share their raw data to learn a model of good quality. One scenario is to recommend items to clients with limited historical data and sharing similar preferences with other clients in a social network. On the other hand, due to the increasing demands for the protection of clients' data privacy, Federated Learning (FL) has been widely adopted: FL requires models to be trained in a multi-client system and restricts sharing of raw data among clients. The underlying potential data-sharing conflict between LoG and FL is under-explored and how to benefit from both sides is a promising problem. In this work, we first formulate the Graph Federated Learning (GFL) problem that unifies LoG and FL in multi-client systems and then propose sharing hidden representation instead of the raw data of neighbors to protect data privacy as a solution. To overcome the biased gradient problem in GFL, we provide a gradient estimation method and its convergence analysis under the non-convex objective. In experiments, we evaluate our method in classification tasks on graphs. Our experiment shows a good match between our theory and the practice.

==> figures&tables/tablelol.tex <==
\begin{table}[t!]
\caption{\footnotesize Results on the deterministic node classification task. This table provides the results of the average test accuracy and the corresponding $95\%$ confidence interval}
\label{table: DNC_results}
\centering
\vspace{-1.5mm}
\begin{tabular}{ c c c} 
\hline
& Synthetic Graphs & subCora\\
\hline
\texttt{$\text{GAP}_{10}$} & $93.4 \pm 0.99\%$ & $54.1 \pm 3.72\%$\\
\texttt{$\text{GAP}_{20}$} & $93.3 \pm 0.94\%$ & $\boxed{54.3 \pm 3.73\%}$\\
\texttt{$\text{GAP}_{50}$} & $93.0 \pm 0.96\%$ & $54.0 \pm 3.73\%$\\
\texttt{APPNP} & $93.2 \pm 0.92\%$ & $54.2 \pm 3.69\%$\\
\texttt{GCN} & $\boxed{95.2 \pm 0.54\%}$ & $51.9 \pm 3.78\%$\\
\texttt{GAT} & $93.3 \pm 1.03\%$ & $47.9	\pm 3.01\%$\\
\texttt{GraphSAGE} & $70.2 \pm 4.21\%$ & $47.0 \pm 3.73\%$\\
\hline
\end{tabular}
\vspace{-1.5mm}
\end{table}
